OrchestraLLM: Efficient Orchestration of Language Models for Dialogue State Tracking

Large language models (LLMs) have revolutionized the landscape of Natural Language Processing systems, but are computationally expensive. To reduce the cost without sacrificing performance, previous studies have explored various approaches to harness the potential of Small Language Models (SLMs) as cost-effective alternatives to their larger counterparts. Driven by findings that SLMs and LLMs exhibit complementary strengths in a structured knowledge extraction task, this work presents a novel SLM/LLM routing framework designed to improve computational efficiency and enhance task performance. First, exemplar pools are created to represent the types of contexts where each LM provides a more reliable answer, leveraging a sentence embedding fine-tuned so that context similarity is close to dialogue state similarity. Then, during inference, the k-nearest exemplars to the testing instance are retrieved, and the instance is routed according to majority vote. In dialogue state tracking tasks, the proposed routing framework enhances performance substantially compared to relying solely on LLMs, while reducing the computational costs by over 50%.

==> Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}


\newcommand{\R}{\mathbb{R}}

\newcommand{\zeromatrix}{\mathbf{0}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}

\newcommand{\mC}{\mathcal{C}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mR}{\mathcal{R}}

\newcommand{\iL}{\mathit{L}}
\newcommand{\iQ}{\mathit{Q}}
\newcommand{\iR}{\mathit{R}}
\newcommand{\iU}{\mathit{U}}
\newcommand{\iV}{\mathit{V}}
\newcommand{\iX}{\mathit{X}}
\newcommand{\iY}{\mathit{Y}}

\newcommand{\sigmoid}{\text{sigm}}
%\newcommand{\vector}{\text{vec}}
\newcommand{\KL}{\text{KL}}
\newcommand{\Loss}{\mathcal{L}}
% \newcommand{\st}{\text{ s.t. }}

% Objective functions
\newcommand{\bilinear}[3]{#1^{\top}#2#3}
\newcommand{\bidiag}[3]{(#1 \circ #3) ^{\top} #2}
\newcommand{\diag}[1]{\text{diag}\left(#1\right)}
\newcommand{\biband}[3]{#1^{\top}#2#3}

% Dependency paths
\newcommand{\leftarc}[1]{$\leftarrow${[#1]}-}
\newcommand{\rightarc}[1]{-{[#1]}$\rightarrow$}
\newcommand{\wildcard}{$\langle*\rangle$}

\newcommand{\gene}[1]{{\texttt{#1}}}
\newcommand{\rev}[1]{#1$^{-1}$}

\newcommand{\neigh}[1]{\text{nb}\left(#1\right)}
\newcommand{\diagm}[1]{\text{diag}\left(#1\right)}
\newcommand{\ind}[1]{\mathbf{1}\left(#1\right)}
\newcommand{\argmin}[1]{\underset{#1}{\text{argmin}}}
%\newcommand{\vector}[1]{\underset{#1}{\text{vec}}}
\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\bigl(#1\bigr)}}
\newcommand{\cheading}[2]{\textbf{#1\hfill #2}}
\newcommand{\highest}[1]{\textbf{#1}}% == highest score



%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
% \newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\bA}{\mathbb{A}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bJ}{\mathbb{J}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bO}{\mathbb{O}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{{\mathbb{S}}}
\newcommand{\bT}{{\mathbb{T}}}
\newcommand{\bU}{\mathbb{U}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\bZ}{\mathbb{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}


%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\em Proof:\ }}{\hfill\BlackBox\\[.3mm]}
\fi
%\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}[theorem]{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
\newtheorem{claim}[theorem]{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}[theorem]{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%\newcommand{\ln}{\mathop{\mathrm{ln}}}
%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\etc}{\emph{etc.}\ }
\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.,}\ }
\newcommand{\ie}{\emph{i.e.,}\ }
\newcommand{\iid}{\emph{iid}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\rhs}{\text{ r.h.s. }}
\newcommand{\lhs}{\text{ l.h.s. }}

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}
\newcommand{\tauvec}{\vec{\tau}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\ve}{\varepsilon}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}
\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


\newcommand{\Aone}{\textbf{A1}}
\newcommand{\Atwo}{\textbf{A2}}

\newcommand{\Ker}{\ensuremath{\mathrm{Ker}}}
\newcommand{\Img}{\ensuremath{\mathrm{Im}}}

\newcommand{\cvxCondjc}{{\sf cvxCondJC}}
\newcommand{\cvxCond}{{\sf cvxCond}}
\newcommand{\altCondjc}{{\sf altCondJC}}
\newcommand{\altCond}{{\sf altCond}}

\newcommand{\cvxDisc}{{\sf cvxDisc}}
\newcommand{\JB}{{\sf JB}}
\newcommand{\GS}{{\sf GS}}

\newcommand{\cvxJoint}{{\sf cvxJoint}}
\newcommand{\LG}{{\sf LG}}
\newcommand{\NB}{{\sf NB}}

%%%%%%%%%%%%%%%%%%%linear algebra defs%%%%%%%%%%%%%%%
\newcommand{\unifint}{\int^{1}_{0}}


==> Deprecated_Files/crosstask_retriever_mwoz.tex <==
\begin{table}[t]
    \small
    \centering
    \begin{tabular}{l|ccc}
    \toprule
        \textbf{Models}  & \textbf{\textit{Assignment}}  & \textbf{TLB}  & \textbf{DST}\\
        \midrule
        Prompt-DST & N & 73.43 &  46.06  \\
        IC-DST & N & 78.21 & 49.68 \\
        \midrule
       Dual Model & 60\% & 80.74  & 50.19  \\
        task-ware & 61\% & 82.24 & 54.27 \\
        task+expert-aware & 66\% & 81.65 & 52.02 \\
        SGD task-aware & 54\% & 80.75 & 50.21 \\
        \bottomrule
    \end{tabular}
    \caption{Cross task retriever results on MultiWOZ. We denote the \% of testing turns routed to Prompt-DST (SLM) as \textit{Assignment}.}
    \label{tab:crosstask_retriever_mwoz}
\end{table}

==> Deprecated_Files/crosstask_retriever_sgd.tex <==
\begin{table}[t]
    \small
    \centering
    \begin{tabular}{l|ccc}
    \toprule
        \textbf{Models}  & \textbf{\textit{Assignment}}  & \textbf{TLB}  & \textbf{DST}\\
        \midrule
        Prompt-DST & N & 62.21 & 28.38\\
        IC-DST & N & 63.86 & 33.15 \\
        \midrule
       Dual Model & 60\% & 65.97  & 32.75  \\
        task-ware & 61\% & 67.25 & 32.78 \\
        task+expert-aware & 66\% & 68.09 & 33.07 \\
        MWOZ task-aware & 43\% & 66.57 & 33.62 \\
        \bottomrule
    \end{tabular}
    \caption{Cross task retriever results on SGD. We denote the \% of testing turns routed to Prompt-DST (SLM) as \textit{Assignment}.}
    \label{tab:crosstask_retriever_sgd}
\end{table}

==> Deprecated_Files/intro2.tex <==
\section{Introduction}
Large Language Models (LLMs) have emerged as a powerful tool for performing a wide array of tasks. However, they come with increasingly high computational costs as the sizes grow. Because many tasks have computation resource constraints, there is substantial interest in architectures that reduce costs but still take advantage of LLM capabilities.  Conversational systems associated with task-oriented dialogues, such as virtual assistants, typically have such resource constraints.

Task-oriented dialogues involving structured data typically rely on Dialogue State Tracking (DST), where user intent is extracted from the dialogue history between a user and the agent in the form of slot values associated with a predefined schema. Pre-trained language models that are fine-tuned have been used in DST for a few years, including both autoregressive LMs \cite{ham2020end,hosseini2020simple,peng2020soloist} and sequence-to-sequence models \cite{lee2021dialogue,su2022multi,bang-etal-2023-task,imrattanatrai-fukuda-2023-end,wang2023divide}. These methods generally rely on the availability of a substantial training corpus to achieve good performance.

LLMs enable zero-shot or few-shot learning~\cite{brown2020language}. For DST, \citet{xie2022unifiedskg,hudevcek2023large} prompts LLM with human-authored task descriptions or in-context exemplars. 
~\citet{hu-etal-2022-context} improves the in-context learning for DST performance by incorporating a retriever to fetch useful exemplars. ~\citet{king2023diverse} further increases the diversity of in-context exemplars and improves the decoding mechanism. In our work, we seek to take advantage of the effectiveness of LLMs with a small amount of training data but reduce the cost.

%%MO: I don't think that the combinations of LLMs are relevant to this paper, so I'd omit this paragraph
%Recent research endeavors have explored collaborative approaches involving LLMs to enhance task performance. These approaches encompass selecting the most suitable answer from multiple LLM outputs~\cite{si2023mixture}, fusing a set of LLM outputs to generate an improved result~\cite{jiang2023llm}, and orchestrating a sequence of LLMs with an LLM planner~\cite{lu2023chameleon}. However, a drawback of these LLM-centric methods is their high computational cost, posing a significant obstacle to their practical deployment in real-world settings.

To mitigate the computational demands of LLMs in general, cascade-based strategies have been proposed~\cite{chen2023frugalgpt, madaan2023automix} where a query is directed to LLM when it cannot be resolved by Small Language Models (SLMs). However, these approaches invariably introduce latency and computational redundancy since they consistently query SLMs. In an effort to strike a balance between cost reduction and accuracy enhancement, other approaches~\cite{kag2022efficient, vsakota2023fly} use binary classifiers to predict the most appropriate LLM to utilize. However, a limitation of these classifier-based approaches is the necessity for retraining when introducing a new pair of models, limiting the generalization abilities of the system.

In this work, we propose a dynamic framework that leverages small (fine-tuned) and large LM experts. We hypothesize that the SLM fine-tuned on a small amount of data can learn important categorical slot values and task-specific artifacts, while the LLM will be better at handling open-valued slots and more complex queries.
We propose a retrieval-based router that
leverages exemplar pools that represent the types of dialogue contexts where the different LMs provide more reliable answers. The exemplar and input contexts are represented by a sentence embedding that is fine-tuned to drive context similarity to be close to dialogue state similarity.
At inference time, a suitable expert is selected based on the embedding distances between the testing instance and the instances in the expert pools. This removes the need for a new router when a new expert is introduced. Previous studies have explored routing task instances by using off-the-shelf retrievers with dense retrieval to retrieve a relevant expert during inference time~\cite{jang2023exploring}. Their setting focuses on task transfer and requires a batch of testing examples as the query to retrieve an expert for a whole task. However, this approach falls short of generalization to the dynamic and interactive characteristics of dialogue systems. In contrast, our proposed framework retrieves an expert model based on testing instance turn-level characteristics, targeting the optimal expert allocation for turns with diverse attributes.

In summary, the key contribution of this work is the introduction of a novel switching model designed to reduce the computational costs associated with LLMs while simultaneously improving performance. Experimental results on two different multi-domain DST benchmarks (MultiWOZ~\cite{budzianowski2018multiwoz,ye-etal-2022-multiwoz} and SGD~\cite{rastogi2020towards}) demonstrate that \ourmodelshort capitalizes on the proficiencies of different experts, outperforming LLM systems while also achieving a substantial reduction of over 50\% in computational costs.

%%MO: I don't see the localized change argument so left this out. You can put it back if you explain more
%The a SLM is finetuned to specialize in domain-specific knowledge and task-specific artifacts, it is better at grasping localized changes in DST~\cite{xie2022unifiedskg}. 

==> Deprecated_Files/introduction.tex <==
\section{Introduction}
Large Language Models (LLMs) have emerged as the linchpin for performing a wide array of NLP tasks. Recent research endeavors have explored collaborative approaches involving LLMs to enhance task performance. These approaches encompass selecting the most suitable answer from multiple LLM outputs~\cite{si2023mixture}, fusing a set of LLM outputs to generate an improved result~\cite{jiang2023llm}, and orchestrating a sequence of LLMs with an LLM planner~\cite{lu2023xchameleon}. However, a noteworthy drawback of these LLM-centric methods is their voracious appetite for computational resources, posing a significant obstacle to their practical deployment in real-world settings.

To mitigate the computational demands, cascade-based strategies have been proposed~\cite{chen2023frugalgpt, madaan2023automix} where a query is directed to LLM when it cannot be resolved by Small Language Models (SLMs). Nonetheless, these approaches invariably introduce latency and computational redundancy since they consistently query SLMs. In an effort to strike a balance between cost reduction and accuracy enhancement, previous works~\cite{kag2022efficient, vsakota2023fly} have introduced the idea of training binary classifiers to predict the most appropriate LLM to utilize. However, a significant limitation of these classifier-based approaches is the necessity for retraining when introducing a new pair of models, limiting the generalization abilities of the system.\\

In this work, we propose a dynamic framework that simultaneously leverages small and large LM experts along with a retrieval-based router. In inference time, a suitable expert is selected based on the embedding distances between the testing instance and the instances in the expert pools. This removes the need for a new router when a new expert is introduced. Previous studies have explored routing task instances by using off-the-shelf retrievers with dense retrieval to retrieve a relevant expert during inference time~\cite{jang2023exploring}. Their setting focuses on task transfer and requires a batch of testing examples as the query to retrieve an expert for a whole task. However, this approach falls short of generalization to the dynamic and interactive characteristics of dialogue systems. In contrast, our proposed framework retrieves an expert model based on testing instance turn-level semantics, targeting the optimal expert allocation for turns with diverse attributes.

We focus on dialogue state tracking (DST), which extracts user intents from the dialogue history between the user
and the agent in the form of slot values associated with a predefined schema. Intuitively, a SLM is finetuned to specialize in domain-specific knowledge and task-specific artifacts, it is better at grasping localized changes in DST~\cite{xie2022unifiedskg}. On the other hand, a LLM is adept at navigating complex scenarios demanding common sense knowledge or long-context understanding. By capitalizing on the proficiencies of diverse experts, our preliminary studies manifest that \ourmodelshort surpasses the LLM system while also reducing over 50\% computing costs on popular benchmarks, including MultiWOZ~\cite{budzianowski2018multiwoz,ye-etal-2022-multiwoz} and SGD~\cite{rastogi2020towards}.


==> Deprecated_Files/related.tex <==
\section{Related Work}
\subsection{Model Compression}
Model compression primarily falls into three major paradigms: pruning, distillation, and quantization. Pruning strategies are primarily devised to reduce computational overhead by selecting and retaining a subnetwork within a larger model~\cite{fan2019reducing, michel2019sixteen, wang2020structured, lagunas2021block, xia2022structured}. In contrast, distillation techniques entail the training of a compact student model, with the objective of imparting the knowledge and performance of a larger teacher model~\cite{sanh2019distilbert, turc2019well, jiao2020tinybert}. Finally, quantization methods aim to diminish memory demands by representing model parameters with fewer bits, thereby trading off a degree of precision for enhanced efficiency~\cite{shen2020q, dettmers2022llm, dettmers2023qlora}. Note that the aforementioned methods are characterized as "static" in nature, as they primarily focus on the optimization of fixed model architectures for each data point. In contrast, the routing framework introduced in this work adopts a dynamic perspective.

\subsection{Sample-Adaptive Inference}
To enable variable levels of computational resources to be allocated for processing different input samples, two predominant categories of approaches have emerged in this domain: early exiting and token dropping. Early exiting strategies typically incorporate additional classifiers at intermediate layers within a model, determining whether a given input example should terminate its processing prematurely and abstain from propagating to subsequent layers~\cite{liu-etal-2020-fastbert, xin-etal-2021-berxit, zhou2020bert}. On the other hand, token-dropping techniques aim to dynamically reduce the length of the input sequence, achieved by selectively excluding certain tokens from the input sequence, which are subsequently not passed on to subsequent layers in the model~\cite{goyal2020power, guan2022transkimmer, kim-cho-2021-length}. ~\citet{salehi2023sharcs} also studies to direct different samples to sub-networks with varying
widths. Our proposed routing framework also embraces sample-adaptive inference. However, it distinguishes itself by leveraging not just a single model but a combination of models.

\subsection{Model Switching}
There has been a growing body of research focusing on the concept of model switching, wherein input examples are intelligently routed between small and large models based on their individual complexity levels. For instance, ~\citet{madaan2023automix} proposes a methodology that leverages an external meta-verifier to ascertain the correctness of predictions made by a Small Language Model (SLM) and to determine whether an example warrants routing to a Large Language Model (LLM). In contrast, our approach does not necessitate the use of additional verifiers. Another set of related approaches, exemplified by the work of \citet{vsakota2023fly,kag2022efficient}, involves training binary classifiers to categorize examples as suitable for SLM or LLM processing. This approach requires the router to be trained on labeled data where language models have made predictions. In contrast, our methodology exhibits the ability to generalize to unseen combinations of model pairs and tasks, enhancing its versatility.

% \subsection{LLM Collaboration}
% \textbf{Ensemble}
% ~\cite{jang2023exploring}

% \textbf{Agent and Tool Use}
% ~\cite{Chamelon,Reflexion} 




\subsection{LM-centric Dialogue State Tracking}
\textbf{Autoregressive LM}\\
Systems fine-tuned from autoregressive pretrained LMs have been developed~\cite {ham2020end,hosseini2020simple,peng2020soloist}. These systems often do not require task-specific modules but often take additional supervision as inputs. Both \citet{ham2020end} and \citet{hosseini2020simple} require dialogue acts as inputs. Both \citet{hosseini2020simple} and \citet{peng2020soloist} require DB search results as inputs. Our approaches in this thesis require only the previous dialogue states and the associated system response. 

\textbf{Sequence-to-Sequence LM}\\
Systems that are fine-tuned from sequence-to-sequence pretrained LMs have been developed to build multi-tasking dialogue agents, such as state tracking, response generation, and intent detection. ~\citet{bang2023task} utilizes adapters~\cite{houlsby2019parameter} to achieve efficient multi-task learning. ~\citet{imrattanatrai2023end} contextualizes dialogue inputs with schema and associated descriptions. ~\citet{su2022multi} finetunes the LM with additional task descriptions, leveraging the instruction following abilities from T5. ~\citet{wang2023divide} trains experts of the same model architecture with different subsets of data and ensembles the predictions while our approach focuses on leveraging experts with the same set of data and combines the complementary strengths of SLM and LLM. 

\textbf{Large langauge model}\\
LLM (here we refer to models with more than 30B parameters) enables zero-shot or few-shot prompting~\cite{brown2020language}. ~\citet{xie2022unifiedskg,hudevcek2023large} prompts LLM with human-authored task descriptions or in-context exemplars. 
~\citet{hu-etal-2022-context} improves the in-context learning for DST performance by incorporating a retriever to fetch useful exemplars. ~\citet{king2023diverse} further increases the diversity of in-context exemplars and improves the decoding mechanism. 




==> Deprecated_Files/router.tex <==
% \section{An Interactive Framework with Dynamic Routing}
\section{Approach}
In this work, we focus on constructing dialogue states by accumulating TLBs, which allows flexible dynamic routing. In other words, the domain-specific SLM handles most parts of the input dialogue and only defers those difficult turns to the general-purpose LLM for efficiency. 
Here, we present our approach for DST, \ourmodelshort, which achieves effective routing via contrastive learning. 
The overall framework is illustrated in \autoref{fig:system}.
We denote different DST models as \textbf{experts}.
Given a new input instance, \ourmodelshort first compares it with exemplar instances from each \textbf{expert pool} and retrieves top-K exemplars. Following that, the routing is carried out by assigning the input to the most suitable expert based on majority voting routing. We hypothesize that examples with similar semantic embeddings are of the same difficulty level and a suitable expert can thus be selected based on the embedding distances between the input instance and the instances in the expert pools.
In the following, we provide details of how the inputs and expert-pool instances are represented and the corresponding training and inference methods.

\subsection{Routing via Contrastive Learning}
In this part, we present our routing model using contrastive learning.
We develop our routing retriever using a hold-out set consisting of a small number of dialogues, which is also used to construct the expert pool.
Similar to recent work on dense retrieval \cite{karpukhin-etal-2020-dense},
our retriever uses a bi-encoder architecture, which encodes dialogues with labels and predictions into embedding space.
Throughout the work, SenBERT \cite{reimers-2019-sentence-bert} is used as the backbone embedding model.
Here, the routing is carried out at the turn level.
Given the $t$-th turn, the input to the retriever model includes a triplet of $(DST_{t-1}, A_{t-1}, U_t)$.
The retrieval target set consists of similar triplets built from all dialogues from the hold-out set.
% We finetune the retriever model with a contrastive loss so that the similarity between a positive example pair is high and the similarity between a negative example pair is low.

We consider two ways of constructing supervision for training the routing retriever.
\begin{comment}
Turn-level embeddings can be computed with vanilla off-the-shelf sentence embedder, \eg SenBERT . However, these embeddings are too generic for our intended use case. Our goal is to obtain fine-grained task-specific embeddings for a turn pair along with their context history.  
Building on the retriever from IC-DST \cite{hu-etal-2022-context}, we implement a specialized retriever by fine-tuning using a few examples with two types of supervision.  \\
\end{comment}
\paragraph{Task-Aware Supervision.}
Here, we leverage the gold annotations of the hold-out set dialogues for deriving positive and negative sets. 
First, we consider using the similarity of turn changes.
Suppose there are two sets of turn changes, $TLB_\mathit{a}=\{(s_1^a, v_1^a), \cdots, (s_m^a, v_m^a)\}$, $TLB_\mathit{b}=\{(s_1^b, v_1^b), \cdots, (s_n^b, v_n^b)\}$. 
Following \citet{hu-etal-2022-context}, the slot-value pair similarity is 
\begin{align*}
    F_{\mathit{slot\mbox{-}value}} = F(&\{(s_1^a, v_1^a), \cdots,(s_m^a, v_m^a)\},\\
    &\{(s_1^b, v_1^b), \cdots, (s_n^b, v_n^b)\}) .
\end{align*} 
and the slot similarity is
\begin{align*}
    F_{\mathit{slot}} = F(\{s_1^a, \cdots,s_m^a\}, \{s_1^b, \cdots, s_n^b\}).
\end{align*}
where $F$ is the standard definition of F1 score \ie $F=\frac{2PR}{P+R}$, in which $P$ is precision, and $R$ is recall. 
Thus, the similarity score between $TLB_\mathit{a}$ and $TLB_\mathit{b}$ is 
\begin{align*}
Sim(TLB_\mathit{a}, TLB_\mathit{b}) = F_{\mathit{slot\mbox{-}value}} + F_{\mathit{slot}} - 1
\end{align*}

In addition to turn change, context history also plays an important role in determining the difficulty of a particular turn. For example, turns in the later part of a dialogue often refer to previous entities, requiring context understanding to correctly predict the slot and value. 
Assume two sets of accumulated DST in turn $t-1$ are $DST_\mathit{a}^\mathit{{t-1}}=\{(s_1^a, v_1^a), \cdots, (s_m^a, v_m^a)\}^{t-1}$, $DST_\mathit{b}^\mathit{{t-1}}=\{(s_1^b, v_1^b), \cdots, (s_n^b, v_n^b)\}^{t-1}$. Therefore we also consider the context similarity as
\begin{align*}
Sim(DST_\mathit{a}^\mathit{{t-1}}, DST_\mathit{b}^\mathit{{t-1}}) = F_{\mathit{slot\mbox{-}value}} + F_{\mathit{slot}} - 1
\end{align*}

Finally, we combine two similarity scores (measured at turn change and dialogue state respectively) and define the similarity between turn a and turn b as
\begin{align*}
    \frac{1}{2} Sim_{\mathit{context}} + Sim_{\mathit{slot\mbox{-}value}} .
\end{align*}
% \mocomment{It is not obvious what it means to "respect both...". You need to more concretely define this.} 

The positive and negative examples for the training sample are identified by first computing similarity for each sample in the hold-out set.
Then, the $l$ highest and lowest scored samples are used as positive and negative examples, respectively.

\paragraph{Expert-Aware Supervision.}
In addition to acquiring task-aware semantics, we aim to equip our retriever with the ability to discern the expertise of different models across various examples.
Different from task-aware supervision, this requires all experts to perform inference on the set of hold-out dialogues.
Based on the prediction results, each turn can be assigned with an \textbf{expert label}, indicating the most efficient expert that can predict the DST more accurately, \ie accurate smaller models are preferred.
Turns sharing the same expert label are grouped into the corresponding \textbf{expert pool}.
Utilizing an off-the-shelf embedder (\eg SenBERT), we then use every turn in the hold-out set as a query to retrieve the $l$ highest and lowest scored samples.
Note that the same input as task-aware supervision is used here.
Among the top-$l$ samples, only those that share the same expert label with the query sample are retained as positive examples, while those with different labels of the bottom-$l$ set are retained as negative.\\ 
\paragraph{Training.}
The positive and negative examples sourced from task-aware supervision and expert-aware supervision can be used for training individually or collectively.
We finetune the retriever model with a contrastive loss so that the similarity between a positive example pair is high and the similarity between a negative example pair is low. \footnote{In theory, task-aware supervision can be derived from all training dialogues without the need for expert inference. However, in all our experiments, we employ the same set of hold-out dialogues for both task-aware and expert-aware supervision.}

\subsection{Expert Selection by Retrieval}
We now describe how we leverage the task-specialized retriever to route instances during inference. We first construct expert libraries for each expert separately. For each expert, only the examples that are correctly predicted by the expert will be included in the pool.

We then compute cosine similarities between the testing instance and each instance in every expert retrieval pool. We sort all the retrieved instances and take the majority of experts among the top K.
% The intuition behind this method is that the more similar instances this expert specializes in, the more likely this expert is going to make correct predictions on this testing instance. 

Formally, let $R$ be the finetuned embedding model.
For each test example $x$, 
we retrieve the $k$ training examples such that $e_i, e_2, \cdots, e_k$ are the nearest neighbors of $x^*$, given by a the cosine similarity score,
\begin{align*}
    \mathit{score}(x,e) = \text{cos}(R(x), R(e)).
\end{align*}


==> tables/OOD_sgd.tex <==
% \begin{table}[t]
%     \small
%     \centering
%     \begin{tabular}{l|ccc}
%     \toprule
%         \textbf{Models}  & \textbf{\textit{In-Domain}}  & \textbf{\textit{Half OOD}}  & \textbf{\textit{OOD}}\\
%         \midrule
%         Prompt-DST & 62.30 & 24.13 &  25.22  \\
%         IC-DST & 53.29 & 33.67 & 27.07 \\
%         \midrule
%        Dual Model & 62.28 & 30.79  & 28.12  \\
%         task-ware & 64.29 & 29.55 & 29.07 \\
%         task+expert-aware & 62.16 &  30.78 & 28.91 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Cross-domain generalization results on SGD. We denote \textit{In-Domain} when all of the testing domains are in the training set and denote \textit{OOD} when all of the testing domains are not in the training set. For all other dialogues, we categorize them as \textit{Half OOD}. We report DST JGA for all settings.}
%     \label{tab:sgd_generalization}
% \end{table}


\begin{table}[t]
    \small
    \centering
    \begin{tabular}{l|ccc}
    \toprule
        \textbf{Models}  & \textbf{\textit{In-Domain}}  & \textbf{\textit{Half OOD}}  & \textbf{\textit{OOD}}\\
        \midrule
        Prompt-DST & 76.41 & 60.6 &  60.68 \\
        IC-DST & 73.35 & 63.58 & 61.38 \\
        \midrule
       RoutingDST & 79.85 & 64.23  & 64.68  \\
        task-ware & 80.76 & 65.21 & 66.35 \\
        task+expert-aware & 79.82 &  66.72 & 66.89 \\
        \bottomrule
    \end{tabular}
    \caption{Cross-domain generalization results on SGD. We denote \textit{In-Domain} when all of the testing domains are in the training set and denote \textit{OOD} when all of the testing domains are not in the training set. For all other dialogues, we categorize them as \textit{Half OOD}. We report TLB JGA for all settings.}
    \label{tab:sgd_generalization}
\end{table}
